NoRA: A Tensor Network Ansatz for Volume-Law Entangled Equilibrium States of Highly Connected Hamiltonians

Motivated by the ground state structure of quantum models with all-to-all interactions such as mean-field quantum spin glass models and the Sachdev-Ye-Kitaev (SYK) model, we propose a tensor network architecture which can accomodate volume law entanglement and a large ground state degeneracy. We call this architecture the non-local renormalization ansatz (NoRA) because it can be viewed as a generalization of MERA, DMERA, and branching MERA networks with the constraints of spatial locality removed. We argue that the architecture is potentially expressive enough to capture the entanglement and complexity of the ground space of the SYK model, thus making it a suitable variational ansatz, but we leave a detailed study of SYK to future work. We further explore the architecture in the special case in which the tensors are random Clifford gates. Here the architecture can be viewed as the encoding map of a random stabilizer code. We introduce a family of codes inspired by the SYK model which can be chosen to have constant rate and linear distance at the cost of some high weight stabilizers. We also comment on potential similarities between this code family and the approximate code formed from the SYK ground space.

==> old/abstract.tex <==
\begin{abstract}

Motivated by the entanglement structure of all-to-all quantum models like the SYK model and mean-field quantum spin glass models, we propose a tensor network architecture which can capture volume law entanglement and can accommodate a large ground state degeneracy. The architecture can be viewed as a generalization of MERA, DMERA, and branching MERA networks where we remove the constraints of spatial locality. We argue that the proposed architecture can roughly capture the entanglement and complexity of the SYK model, but we leave a more detailed study to future work. We further explore the basic architecture by considering the special case where the tensors are random Clifford gates. In this case, the architecture can generate a stabilizer code with constant rate and distance that approximately saturates the quantum singleton bound, albeit at the cost of some high weight stabilizers.



%Motivated by the approximation of CFTs and their renormalization as MERA tensor networks, we constructed a network whose thermal entropy and complexity scales how one would expect from SYK models and their holographic dual in the JT gravity bulk. Taking the zero-temperature limit, the resulting circuit was interpreted as a quantum error-correcting code which encodes $n_0$ logical qudits in $n = n_0 + 2^{\ell}$ physical qubits where $\ell$ is the number of randomly sampled scrambling layers with depth $D$ in the code. Choosing $n_0 = 2$ and varying $\ell$ and $D$ let us approximate the scaling of the code distance. Unfortunately, due to time constraints only an analysis of the weight evolution for the circuit was available at time of publication. 

%Additionally, we considered the distribution of GHZ states for randomly sampled tripartite Clifford stabilizer states with various qudit dimensions and number $n_{\text{party}}$ of qudits per party. Although we arrived at the expected conclusion that for larger $n$ the GHZ content is of order $\mathcal{O}(1)$ and and thus tends to descrease relative to an increasing $n_{\text{party}}$, some numerical anomalies suggest that a closer inspection of the problem is necessary.
\end{abstract}

==> old/ack.tex <==
\section{Acknowledgements}

==> old/conclusion.tex <==
\section{Conclusion \& Outlook}

Over the course of this work, we have outlined some important aspects and properties of the stabilizer formalism and how one can use it to describe and simulate the scrambling and entanglement of quantum information in different ways. Even though time constraints didn't permit us to do a full analysis of all quantities of interest (especially the code distance of the SYK code), we managed to confirm that our implementation of a stabilizer simulation using random Clifford gates seems to work as intended, and efficiently so.

Some of the next steps to be taken include refining the simulation further and introducing unit testing such that the correctness of the code can be ensured at all times. If interest from outside exists, then a documented API could also be provided in the future. In addition to that, a more systematic analysis of the parameter space for the models of interest has high priority, so that it becomes possible to answer some of the lingering questions outlined in the previous section. But thanks to the generality of the simulation, all kinds of different models can be easily implemented and analysed.



==> old/error_correction.tex <==
\section{Quantum Error Correction}
\label{section:disc}

\subsection{Stabilizer Codes}
\label{sec:stab}

A (quantum) stabilizer code $[[n, k, d]]$ that encodes $k$ physical qudits into $n$ physical qudits with code distance $d$ is defined in terms of a \emph{stabilizer group} $S$, which is an abelian subgroup of the Pauli group $P_n(d)$ i.e.\ the group generated by all possible $n$-element tensor products of the Pauli operators ($d = 2$)
\begin{equation}
    X = \begin{pmatrix}
        0 & 1 \\ 1 & 0
    \end{pmatrix}, \,
    Y = \begin{pmatrix}
        0 & -i \\ i & 0
    \end{pmatrix}, \,
    Z = \begin{pmatrix}
        1 & 0 \\ 0 & -1
    \end{pmatrix}
\end{equation}
or their higher-dimensional counterparts ($d > 2$), which are defined in section \ref{sec:weyl_rep} \cite{qldpc}. The stabilizer group must therefore be generated by $(n - k)$ independent elements of $P_n$. A \emph{code word} is a state vector $\ket{\psi} \in \mathbb{C}^{d^n}$\ footnote{$d$ here is the dimension of the Hilbert space of a single qudit and not the code distance.} that satisfies $s \ket{\psi} = \ket{\psi}$ for all $s \in S$. The space spanned by all possible code words is called the \emph{code space} and has dimension $k$. The operators mapping logical states to other logical states are called \emph{logical operators} and must therefore commute with all elements of the stabilizer group.

Some important quantities in relation to stabilizer codes are
\begin{itemize}
    \item \textbf{operator weight:} The number of elements of $P_1(d)$ in the tensor product of the operator that are not proportional to the identity operator $I$.
    \item \textbf{code weight:} The largest weight an element of the corresponding stabilizer group exhibits.
    \item \textbf{code distance:} The minimal weight of all non-trivial logical operators. Equivalently it can be defined as the minimum number of qudits that have to be changed to arrive at another code word.
\end{itemize}
A \emph{quantum low-density-parity-check} (qLDPC) code is a code with constant weight, regardless of the code length $n$. This means that each stabilizer only acts on a constant number of qudits and each qudit is acted on by only a constant number of stabilizer elements. A \emph{good} qLDPC code has its code space dimension $k$ and distance $d$ scale linearly with the length $n$.

\subsection{Decoupling \& Code Distance}

Determining the distance for a stabilizer code and how it scales with the number of physical qudits is not a trivial thing to do. We present here one way, called the \emph{adversarial approach}, which makes use of analysing the mutual information
\begin{equation}
\label{eq:mut_inf}
    I(A, R) = S(A) + S(R) - S(AR)
\end{equation}
between all possible subsystems $A$ of the physical qudits and some external adversary $R$ who is initially maximally entangled with the code word. A depiction of the setup can be found in figure \ref{fig:decoupling}.
\begin{figure}[hbt]
    \centering
    \tikzfig{figures/decoupling}
    \caption{Circuit representation of the adversarial approach for determining the distance of a stabilizer code. Here $U_{MN}$ is a unitary that takes states of the form $\ket{\psi_{\text{anc}}}_M \otimes \ket{\psi_{\text{code}}}_N$ and maps $\ket{\psi_{\text{code}}}$ to the code space of the chosen stabilizer state. $\ket{\psi_{\text{anc}}}$ is an arbitrary state of ancilla qudits and can therefore be ignored. The code distance is then one less than the size of the smallest choice for $A$ that has non-vanishing mutual information $I(A, R)$ with $R$. The interpretation is that $R$ then has access to enough qudits such that they can change the initial code word.}
    \label{fig:decoupling}
\end{figure}

As can be seen there, $R$ remains maximally entangled with the logical state $\ket{\psi_{\text{code}}}$ even after it has been encoded into the code space by an appropiate unitary $U_{MN}$. The question is therefore what the minimum number of physical qudits $A$ is that the adversary $R$ has to \enquote{steal} to get access to one logical qudit, thus being able to change it. A measure that indicates for which choices of $A$ this is the case is the aforemention mutual information \eqref{eq:mut_inf}, which becomes non-zero in such a case. In that case one says that $A$ is \emph{decoupled} from the rest of the physical qudit space, meaning that the state can be written as a tensor product on $A$ and its complement $MN / A$. The code distance is therefore
\begin{equation}
    d = |A^*| - 1,
\end{equation}
where $A^*$ is the smallest set of physical qudits which satisfies $I(A^*, R) \neq 0$. Since the code word is assumed to be maximally entangled with $R$, this statement is true for all possible choices of $\ket{\psi_{\text{code}}}$.

Implementing this approach as an algorithm is problematic though since iterating about all possible choices for $A$ is combinatorically intensive. A way to simplify the procdeure at the cost of only getting an upper bound approximation for the code distance is by randomly sampling choices for A and determining the smallest one which has non-vanishing mutual information.

==> old/introduction.tex <==
\section{Introduction}
\label{sec:intro}

In recent years, quantum information theory and more specifically quantum error correction have quickly become some of the most-studied subjects in both experimental and theoretical phsyics. This is not only because of the anticipated advent of large-scale quantum computing devices and with them the need for efficient and scalable protection against noise, but also the uncovered connections between certain gravitational and quantum mechanical systems \cite{Maldacena_1999}. Further work on what is now called the AdS/CFT correspondence suggests that maybe even the universe itself exhibits some form of fundamental self-correcting properties in the form of \emph{holography} \cite{Harlow_2016}. 

But while methods to prevent data corruption due to outside noise have long been a staple in modern computer science and are nowadays used in almost all computational devices, trying to accomplish the same for quantum systems is still a relatively new field of research \cite{shor} \cite{gottesmann}. While many concept can indeed be taken from previous work, translating error correction to quantum systems poses a couple of problems that are not present in the classical counterpart. One major issue is that many classical codes employ some form of redundancy to make the information safe against noise. This is not feasible for their quantum analogue as quantum mechanics forbids the cloning of quantum information and manually preparing copies of states is not an efficient method. Additionally, the most naive way of checking if an error occured would involve having to measure the current state of the quantum computer, thus completely or at least partially collapsing the wavefunction and destroying the superpositions.

While a solution to these problems has been found in \emph{stabilizer codes} \cite{gottesmann}, it is not entirely clear yet what kind of codes are feasible and scale well with the system size and the number of qudits one wants to encode. Recent advances \cite{Panteleev_2022} seem to have proven though that there exist so-called \enquote{good} quantum low-density-parity-check (LDPC) codes whose distance scales almost with the system size. This would mean a serious step towards large-scale quantum error correction and bring us towards the cutting edge of classical computer science, where good LDPC codes are nowadays used in a lot of devices.

In this paper we try to set the groundwork for evaluating if such a (good) qLDPC code is realized by the Sachdev-Ye-Kitaev (SYK) model, a system of Majorana fermions with randomly distributed interaction coefficients. Given that the model indeed exhibits error-correcting properties (which is thought to be the case \cite{syk_qec}), we expect that the corresponding code might be LDPC because the defining Hamiltonian has low operator weight. But what makes this model also interesting is that it exhibits an almost conformal symmetry in certain limits and is dual to 2-dimensional Jackiw-Teitelboim (JT) gravity, which is one of the simplest and most well-understood examples for AdS/CFT. If the model therefore can correct errors, this should also be the case for the gravity side of the duality. To explore this idea we constructed a MERA-like tensor network that exhibits some important properties of SYK and tested it for its error correction capabilities.

On a side note, we also employed the phase space formalism reviewed in this paper to evaluate the entanglement content of tripartite Clifford stabilizer states. Considerations from stabilizer tensor networks and AdS/CFT lead to the popular lore that the entanglement content of holographic spacetimes should be dominated by bipartite entanglement. This is because in the ER=EPR picture the wormholes related to tri- or multipartite entanglement are not classical solutions of general relativity and are therefore suppressed by the gravitational path integral \cite{Balasubramanian_2014} \cite{susskind2014}.
Usually those considerations are made for a large number of qudits as we naturally expect the Hilbert space of the bulk/boundary to be unimagineable in size. But it is also of interest for us if similar statements can be made for systems where the number of qudits is more manageable (e.g.\ condensed matter systems or quantum computers).

==> old/results.tex <==
\section{Results}

\subsection{Technical Details}
The stabilizer simulation used to generate the following data was written in Python 3.9.7 using Numpy 1.21 (linear algebra) \cite{harris2020array} and Galois 0.0.24 (finite field arithmetic) \cite{Hostetter_Galois_2020}, and is based on the projective symplectic representation discussed in section \ref{sec:phase_space}. The algorithm used to randomly sample symplectic matrices for Clifford operators is based on \cite{Koenig_2014}, but was generalized to work for any choice of prime qudit dimension $d$. The complete code can be found at
\\~\\
\centerline{\url{https://github.com/Slartibartfass42/ldpc_syk}.}
\\~\\
All data in this paper was generated using a 2021 MacBook Pro with M1 Pro processor and 16 GB RAM. If the computation involved random sampling, an average over 1000 iterations is displayed together with the error on the mean\footnote{Some errors are so small that they are not visible in the figures.}.

\subsection{Simple Scrambling}

We first considered the simple case of the two-site wall scrambling circuit as depicted in figure \ref{fig:wall_circuit}, except that we randomly chose the Weyl pairs that the random Cliffords act on at each step in the process. The system therefore does no exhibit a causal cone. Analysing the weight evolution of such a circuit provides a good heuristic for how quickly such a system becomes highly entangled and thus chaotic.

Starting with unit weight $d=3$ Weyl operators acting on $n = 2^1, 2^2, \ldots, 2^7$ sites, we recorded their new weight after each scrambling layer until the system equilibrated around some value. We call the average step number when this happens the \emph{scrambling time} $T^*$. The resuling weight evolution over time $T$ (i.e.\ the number of steps) is depicted in figure \ref{fig:simple_weights}.
\begin{figure}[hbt]
    \centering
    \includegraphics[width=.9\linewidth]{figures/simple_weights.png}
    \caption{The average weight evolution of $n$ Weyl operators ($d=3$) with initial unit weight overall when subjugated to repeated random two-site scrambling Clifford gates as seen in figure \ref{fig:wall_circuit}. The dashed lines indicate the expected values the weights approach over time, namely $8n/9$. This is because a single randomly sampled $d=3$ Weyl operator has a chance of $8/9$ to have a non-zero weight i.e.\ not being the identity operator.}
    \label{fig:simple_weights}
\end{figure}

We can infer two facts about the scrambling behavior from this graph:
\begin{enumerate}
    \item The initial weight growth $W(T)$ up until the scrambling time is roughly exponential, since it is linear in the logarithmic plot. We can therefore write
    \begin{equation}
        W(T) \sim r^T, \quad T < T^*
    \end{equation}
    for some (numerically determined) constant $r$. We expect $r$ to be slightly less than 2, as that is the number of sites involved in a single scrambling. 

    \item The average weight in equilibrium is not exactly $n$, but $8/9 \cdot n$. This is because a randomly sampled single Weyl operator with $d = 3$ only has a chance of 1 in $9 = d^2$ to have zero weight, namely when it is the identity. This can be seen from \eqref{eq:weyl_single}. In general, the average equilibrium weight of $n$ Weyl operators with qudit dimension $d$ is
    \begin{equation}
        W(T) \sim \frac{d^2 - 1}{d^2} \cdot n, \quad T > T^*.
    \end{equation}
    We also refer to (Weyl) operators in general as being \emph{f-scrambled} if their weight satisfies $W(T) \sim f \cdot n$ after the scrambling time.
\end{enumerate}

Combining these two results we deduce that $r^{T^*} \sim f \cdot n$ for some constants $r$ and $f$, which allows us to approximate the scrambling time as
\begin{equation}
\label{eq:scrm_time}
    T^* \sim \frac{\log(f \cdot n)}{\log(r)}.
\end{equation}
To confirm this statement, we extracted the scrambling times from figure \ref{fig:simple_weights} by manually pinpointing the step when the system seems to reach equilibrium and assuming a human error of $\pm 1$ steps. Plotting those values against the system size and making a fit by using \eqref{eq:scrm_time} resulted in \ref{fig:simple_scrm_time}.
\begin{figure}[hbt]
    \centering
    \includegraphics[width=.9\linewidth]{figures/simple_times.png}
    \caption{The scrambling time $T^*$ with regard to the systems size i.e.\ the number of Weyl operators being scrambled. As expected, the growth follows a logarithmic trend determined by $T^* \sim \log(f n) / \log(r)$ with $r = 1.83 \pm 0.08$ being close to 2. Unlike expected however, the determined value for $f$ differs from the expected value of $8/9$ by $2.09 \sigma$ with $\sigma = 10.72$ being a large error. This is attributed to a systematic error that occurred when determining the scrambling times by hand.}
    \label{fig:simple_scrm_time}
\end{figure}

While the data does indeed seem to follow the trend dictated by our approximation of the scrambling time and with a reasonable result for $r$, the fit for $f$ on the other hand is not quite compatible with the expected value. This is very likely due to how the data points and their errors were determined. Follow-up work on this subject will require a more systematic way of extracting the scrambling time from data such that human bias does not interfere significantly.

\subsection{SYK-Like Scrambling}

Building on top of the previous results, an analogous weight analysis for the SYK circuit seen in figure \ref{fig:syk_circuit} with $d=3$ was performed. Setting $n_{\text{code}} = 2$ and $\ell = 10$, we prepared a Weyl operator with unit weight in the code subsystem and simulated its evolution for varying scrambling circuit depths $D = 1, 2, \ldots 7$. The weight of the operator at each step of the simulation is shown in figure \ref{fig:syk_weights_l10}.
\begin{figure}[hbt]
    \centering
    \includegraphics[width=.9\linewidth]{figures/syk_weights_l10.png}
    \caption{The weight evolution of the SYK circuit as depicted in figure \ref{fig:syk_circuit} for $n_{\text{code}} = 2$, $\ell = 10$ and circuit depth $D = 1, 2, \ldots, 7$. Even for small choices of $D$ the operator weight quickly converges towards the exponentially increasing maximal threshold determined by \eqref{eq:syk_weight_max} (the blue line).}
    \label{fig:syk_weights_l10}
\end{figure}

As can be easily seen, for increasing $D$ the weights at each step $T$ seem to quickly converge towards the predicted average maximum, which is in general given by
\begin{equation}
\label{eq:syk_weight_max}
    W_{\text{max}}(T) = \frac{(d^2 - 1)}{d^2} (n_{\text{code}}+ 2^T), \quad T = 1, 2, \ldots, \ell.
\end{equation}
Note that $D$ is roughly the equivalent of $T$ for the circuit in the previous section section. We therefore denote $D^*(T)$ as the smallest circuit depth for which the system reaches (almost) maximal weight \eqref{eq:syk_weight_max} for each $T$. By looking at figure \ref{fig:syk_weight_diff_l10} this seems universially to be the case for $D^* = 5$, independent of $T$, but $D^* = 4$ seems to give the same result for $T > 1$. For determining the optimal code distance, we therefore suggest to choose $D=4$ for all steps and increase if necessary. Since this behavior should stay roughly the same for larger $\ell$ due to the self-similar nature of the code, $D=4$ might prove to be a good choice for larger system sizes, although that remains to be shown explicitly

\begin{figure}[hbt]
    \centering
    \includegraphics[width=.9\linewidth]{figures/syk_weight_diff_l10.png}
    \caption{The relative weight difference between the simulated and expected values using the same data as in figure \ref{fig:syk_weights_l10}. While  the discrapancy for smaller scrambling depths seems to get larger over time, starting with $D=3$ the difference seems to stay constantly small. Note theat the irregular behaviour for $T < 2$ is likely due to the choice of giving the initial state unit weight.}
    \label{fig:syk_weight_diff_l10}
\end{figure}

Unfortunately, due to time constraints no data regarding the (adversarial) distance of the SYK code has been generated as of writing. We can therefore not say yet if our construction has good error-correcting properties or if it even has the properties of a quantum ldpc code. This will be explored in future work.

\subsection{Tripartite Entanglement}

Last but not least, we considered the GHZ content of tripartite states with $n_{\text{party}} = 1, 2, \ldots, 5$ and $d = 3, 5, 7, 11, 13$. The ration between the average number of GHZ states and $n_{\text{party}}$ is displayed in figure \ref{fig:tripartite_g}.
\begin{figure}[hbt]
    \centering
    \includegraphics[width=.9\linewidth]{figures/tripartite_g.png}
    \caption{Rate of occurrence of tripartite entanglement in form of GHZ states for different systems sizes per party and qudit dimensions. While a general downward trend is visible and expected, the dependence of the ratio on $d$ and $n_{\text{party}}$ is still for the most part unexplained and requires a more extensive analsysis of all quantities involved and the correctness of the simulation.} 
    \label{fig:tripartite_g}
\end{figure}

While the case of $n_{\text{party}} = 1$ does have a significant amount of tripartite entanglement for all $d$, this ratio drops rapidly for $n_{\text{party}} > 1$ and seems to indicate the beginning of a general downward trend that continues even beyond the available data. How exactly this trend behaves requires a more thorough analysis using larger values of $n_{\text{party}}$.

What's interesting is the difference in $d$-dependent behavior for different choices of $n_{\text{party}}$. While for $n_{\text{party}} = 3, 5$ the GHZ content seems to be the same for all qudit dimensions and with vanishing error on the mean, the content for $n_{\text{party}} = 1, 3, 5$ either increases or decreases with larger $d$ while also exhibiting a larger error. So far it reamins unclear if this behavior can be somehow explained, or if it is due to some numerical anomaly or faulty behavior in the stabilizer simulation. More work is therefore necessary.

What might have an explanation though is the oscillating maximum GHZ ratio between even and odd $n_{\text{party}}$. Reminding ourselves that $S(A) + S(B) + S(C) = 2(a + b + c) + 3g$, it is easy to see that if the left-hand side is overall odd, then we must have $g > 0$. This might be more likely to be the case for $n_{\text{party}}$ odd since in the even case the qubits for a single party are on average either pairwise (maximally) entangled with each other or entangled with qubits from other parties. Since that entanglement always comes in pairs the local entropies must be even on average, therfore allowing $g = 0$. This is only specualation though, and an analysis of the local entropies is required to bring certainty.



==> old/syk.tex <==
\section{Motivating the SYK Code}
\label{section:syk}

\subsection{The SYK Model}

As is well known \cite{Maldacena_2016}, the SYK model consists of $N$ Majorana fermions $\psi_i$ which have their dynamics determinded by the Hamiltonian
\begin{equation}
    H = (i)^{q/2} \sum_{1 \leq i_1 \leq i_2 \leq \ldots \leq i_q \leq N} j_{i_1 i_2 \ldots i_q} \psi_{i_1} \psi_{i_2} \ldots \psi_{i_q},
\end{equation}
where $q$ is an even number. The power of $i$ is necessary to ensure that $H$ is hermitean if $q = 2 \mod{4}$. This implies that the system is not symmetric under time reversal if $q/2$ is odd. If one therefore restricts themselves to the time reversal symmetric case, then the case $q=4$ dominates the interactions at low energy. 

Additionally, the coefficients $j_{i_1 i_2 \ldots i_q}$ are drawn from a random Gaussian distribution of real-valued variables such that they have zero mean and variance
\begin{equation}
    \braket{j^2_{i_1, i_2, \ldots, i_q}} = \frac{J^2 (q-1)!}{N^{q-1}},
\end{equation}
where $J$ is a scalar which is taken to be the same for all coefficients. The additonal factors involving $q$ and $N$ are chosen such that it simplifies the large $N$ limit.

\subsection{The MERA Tensor Network}

An important property of the SYK model is that it becomes approximately conformal in the large $N$ limit, which is the reason why AdS/CFT tells us that it is dual to JT gravity. But this connection between SYK models and CFTs is also interesting since the latter can be approximated as a MERA tensor network. One can therefore ask if something similar can be done for SYK models in general.

Looking at an example for a MERA network in figure \ref{fig:mera} it is clear that the circuit exhibits some form of self-similarity. This is necessary to ensure the field theory being approximated is renormalizable. A fine graining from the top of the circuit towards the bottom is also noticeable and can be interepreted as some code space with small Hilbert space dimension being encoded in a larger system of physical qudits. Since this is what we want to achieve, the SYK circuit has to obey these heuritic properties as well.
\begin{figure}[hbt]
    \centering
    \includegraphics[width=.9\linewidth]{figures/mera.png}
    \caption{A visual representation of a MERA tensor network approximating a conformal field theory \cite{Bao_2015}. The triangles and squares can be thought of as creating entanglement and fine-graining the encoded information (by adding more ancillary states) respectively when looked at from the moving-up perspective. Because of the structure of the circuit the information can't distribute faster than indicated by the causal cone (shaded in red).} 
    \label{fig:mera}
\end{figure}

Another important property is the scaling of the (thermodynamic) entropy with the temperature $T$ when an IR cutoff scale $\Lambda$\footnote{This can be interpreted as \enquote{cuting off} all the lower layers of the tensor network starting from a certain layer.} is introduced. In the case of the MERA network this scaling is given by
\begin{equation}
\label{eq:mera_scaling}
    S_{\text{th}} \sim \frac{n}{2^{\ell}} \sim n \left(\frac{T}{\Lambda}\right)^{\#},
\end{equation}
where $n$ is the number of qudits on the lowest layer and $\ell$ is the number of layers remaining after the cutoff. The latter can be found to be
\begin{equation}
\label{eq:layers}
    \ell = \log_2\left( \frac{\Lambda}{T} \right),
\end{equation}
which leads to the second expression in \eqref{eq:mera_scaling} ($\#$ is just an unspecified exponent).

\subsection{The SYK-Inspired Tensor Network Code}

\begin{equation}
    \widetilde{Z}_{\ell, i} = U_{\ell} \, Z_i \, U^{\dagger}_{\ell}
\end{equation}

\begin{equation}
    \Pi_{\ell, i} = I - \widetilde{Z}_{\ell, i}
\end{equation}

\begin{equation}
    \Pi_{\ell} = \bigotimes_{i = 1}^{2^{\ell}} \Pi_{\ell, i}
\end{equation}




\subsection*{OLD}

The task is now to construct a tensor network model that has approximately the same properties as its MERA counterpart, but with the correct scalings for the thermal entropy (and complexity) as expected from estimates for SYK and JT gravity \cite{Brown_2019}. We propose that such a network is given by the circuit in figure \ref{fig:syk_circuit}, where each unitary is modeled by a scrambling circuit with depth $D$ as seen in \ref{fig:wall_circuit}. 
\begin{figure}[hbt]
    \centering
    \tikzfig{figures/syk_circuit}
    \caption{The SYK tensor network taking a code word $\ket{\psi_{\text{code}}}$ and $n_{\text{anc}}$ ancilla qudits and scarmabling them into a system of physical qudits $\ket{\Psi_{\text{phys}}}$. We assume that for this paper that we have $n_{\text{anc}} = 2^{\ell}$ such that all input qudits experience some scrambling in the end. The scrambling unitary at each step is of the form depicted in figure \ref{fig:wall_circuit}.} 
    \label{fig:syk_circuit}
\end{figure}

Assuming an IR cutoff was already performed at the lowest level, $\ell$ is again the number of layers in the circuit and also determined by \eqref{eq:layers}. Self-similarity is then achieved if one sets $n_{\text{anc}} = 2^{\ell}$. Going upwards from the bottom the information is here too entangled by the unitaries and fine-grained due to the stepwise addition of new ancillary states.

\begin{figure}[hbt]
    \centering
    \tikzfig{figures/wall_circuit}
    \caption{An example quantum circuit with depth $D = 5$ used to simulate the rapid scrambling of quantum information. Each gate represents a randomly sampled unitary operator acting on two qudits. If the circuit wires are fixed then this code also exhibits some form of causal cone. But one can also randomly choose which pairs of qudits to scramble at each layer of the circuit.}
    \label{fig:wall_circuit}
\end{figure}

What remains to be checked is the scaling of the entropy, which can be easily seen to satisfy
\begin{equation}
    S_{\text{th}} \sim n_{\text{code}} + \frac{n}{k^{\ell}} \sim n_{\text{code}} + n_{\text{anc}} \left(\frac{T}{\Lambda}\right)^{\#},
\end{equation}
which is similar to what one would expect according to \cite{Brown_2019} \cite{Brown_2016}. We therefore argue that the network shown in \ref{fig:syk_circuit} does indeed satisfy the requirements for modelling a SYK system.


